Multi-Agent Collaboration via Reward Attribution Decomposition

Recent advances in multi-agent reinforcement learning (MARL) have achieved super-human performance in games like Quake 3 and Dota 2. Unfortunately, these techniques require orders-of-magnitude more training rounds than humans and don't generalize to new agent configurations even on the same game. In this work, we propose Collaborative Q-learning (CollaQ) that achieves state-of-the-art performance in the StarCraft multi-agent challenge and supports ad hoc team play. We first formulate multi-agent collaboration as a joint optimization on reward assignment and show that each agent has an approximately optimal policy that decomposes into two parts: one part that only relies on the agent's own state, and the other part that is related to states of nearby agents. Following this novel finding, CollaQ decomposes the Q-function of each agent into a self term and an interactive term, with a Multi-Agent Reward Attribution (MARA) loss that regularizes the training. CollaQ is evaluated on various StarCraft maps and shows that it outperforms existing state-of-the-art techniques (i.e., QMIX, QTRAN, and VDN) by improving the win rate by 40% with the same number of samples. In the more challenging ad hoc team play setting (i.e., reweight/add/remove units without re-training or finetuning), CollaQ outperforms previous SoTA by over 30%.

==> broad_impact.tex <==
\section{Broader Impact}
\vspace{-1mm}
% impact of the work
DRL has shown great performance in many real-world applications including autonomous driving and robotic manipulation. 
But in reality, many deployment scenarios are rather complex and they require multiple intelligent agents that can learn to collaborate with each other.
Examples include multi-player games, multi-robots, cellular antenna tilt control, traffic control systems, smart power grids to network management.
Typically agents in these systems have different knowledge and capabilities.
%with different skills forming a team and collaborating with each other.

Ad-hoc MARL enables agents in such system to efficiently collaborate with new team members (introducing new agent types and changing team sizes) without any retraining or finetuning.
Such modeling would greatly improve the resiliency and robustness of the agents.
Now agents can adapt their behaviors to the change of teammates when deployed in practice.
This is also very important for addressing privacy issues for training agents.
With Ad-hoc MARL, agents can be trained independently from different institutions and still collaborate efficiently together. 
In this way, institutions won't need to give away confidential information/specifications about their agents in order to cooperate.
We believe that Ad-hoc MARL algorithms like \ours{} improves the resiliency of the agent and enables privacy in training such agents.

% limitation and future
Still, most of the studies of Ad-hoc MARL is limited to complex games like Dota 2 and StarCraft, it is far from applying such setting in the real world.
Future researches in building realistic environments, adapting agents' behaviors to humans, or applying Ad-hoc MARL algorithms to real-world applications are essential for the success of Ad-hoc MARL.
